POODLE: Improving Few-shot Learning via Penalizing Out-of-Distribution Samples

In this work, we propose to use out-of-distribution samples, i.e., unlabeled samples coming from outside the target classes, to improve few-shot learning. Specifically, we exploit the easily available out-of-distribution samples to drive the classifier to avoid irrelevant features by maximizing the distance from prototypes to out-of-distribution samples while minimizing that of in-distribution samples (i.e., support, query data). Our approach is simple to implement, agnostic to feature extractors, lightweight without any additional cost for pre-training, and applicable to both inductive and transductive settings. Extensive experiments on various standard benchmarks demonstrate that the proposed method consistently improves the performance of pretrained networks with different architectures.

==> 3_experiments.tex <==
\section{Experiments}

    \textbf{Hyperparameters: } To keep our experiments as simple as possible, \textbf{our hyperparameters are kept fixed across all the experiments and methods (TIM-GD and TIM-ADM)}. The conditional entropy weight $\alpha$ and the cross-entropy weights $\lambda$ in Objective (\ref{eq:tim_objective}) are both set to $0.1$. The temperature parameter $\tau$ in the classifier is set to 15. 
    % In supp. material, however, we show that tuning $\tau$ and $\lambda$ on the validation set can further improve the performance. 
    In our TIM-GD method, we use the ADAM optimizer with the recommended parameters \cite{kingma2014adam}, and run 1000 iterations for each task. For TIM-ADM, we run 150 iterations.
    
    \textbf{Base-training procedure:} The feature extractors are trained following the same simple base-training procedure as in \cite{Laplacian} and using standard networks (ResNet-18 and WRN28-10), for all the experiments. Specifically, they are trained using the standard cross-entropy loss on the base classes, with label smoothing. The label-smoothing parameter is set to 0.1. We emphasize that base training does not involve any meta-learning or episodic training strategy. The models are trained for 90 epochs, with the learning rate initialized to 0.1, and divided by 10 at epochs 45 and 66. Batch size is set to 256 for ResNet-18, and to 128 for WRN28-10. During training, all the images are resized to $84 \times 84$, and we used the same data augmentation procedure as in \cite{Laplacian}, which includes random cropping, color jitter  and random horizontal flipping. 

    \textbf{Datasets: } We resort to 3 few-shot learning  datasets to benchmark the proposed models. As standard few-shot benchmarks, we use the \textbf{\textit{mini}-Imagenet} \cite{matching_net} dataset, with 100 classes split as in \cite{ravi2016optimization}, the \textbf{Caltech-UCSD Birds 200} \cite{cub} (CUB) dataset, with 200 classes, split following \cite{closer_look}, and finally the larger \textbf{\textit{tiered}-Imagenet} dataset, with 608 classes split as in \cite{tiered_imagenet}.
    % Finally, we used the challenging and more realistic \textbf{meta-iNat} dataset \cite{inat}, with 908 classes and severe class imbalance, split according to \cite{inat_benchmark}.

    \subsection{Comparison to state-of-the-art}\label{sec:benchmark}

        We first evaluate our methods TIM-GD and TIM-ADM on the widely adopted \textit{mini}-ImageNet, \textit{tiered}-ImageNet and \textit{CUB} benchmark datasets, in the most common 1-shot 5-way and 5-shot 5-way scenarios, with 15 query shots for each class. Results are reported in \autoref{tab:benchmark_results}, and are averaged over 10,000 episodes, following \cite{simpleshot}. We can observe that both TIM-GD and TIM-ADM yield state-of-the-art performances, consistently across all standard datasets, scenarios and backbones, improving over both transductive and inductive methods, by significant margins. 
        % In supp. material, we further show the superiority of our methods in the 10 and 20-way s
        %and outperforming the best performing methods by over $5\%$ in the 1-shot setting.
        %and $4\%$ on 5-shot tasks.
        
        \begin{table}
        \centering
        \small
        \caption{Comparison to the state-of-the-art methods on \textit{mini}-ImageNet, \textit{tiered}-Imagenet and CUB. The methods are sub-grouped into transductive and inductive methods, as well as by backbone architecture. Our results (gray-shaded) are averaged over 10,000 episodes. "-" signifies the result is unavailable.}
        \begin{tabular}{lccccccccc}
            & & &\multicolumn{2}{c}{\textbf{\textit{mini}-ImageNet}} & \multicolumn{2}{c}{\textbf{\textit{tiered}-ImageNet}} & \multicolumn{2}{c}{\textbf{CUB}} \\
             Method & Transd. & Backbone & 1-shot & 5-shot & 1-shot & 5-shot & 1-shot & 5-shot\\
             \toprule
             MAML \cite{maml}& \multirow{9}{*}{\xmark} & ResNet-18 & 49.6 & 65.7 & - & - & 68.4 & 83.5 \\
            %  Baseline++ \cite{closer_look}& & ResNet-18 & 51.9 & 75.7 & - & - \\
             RelatNet \cite{relation_net}& & ResNet-18 & 52.5 & 69.8 &  - & - & 68.6 & 84.0 \\
             MatchNet \cite{matching_net}& & ResNet-18 & 52.9 & 68.9 &  - & - & 73.5 & 84.5 \\
             ProtoNet \cite{prototypical_nets}& & ResNet-18 & 54.2 & 73.4 &  - & - & 73.0 & 86.6 \\
            %  TADAM \cite{tadam} & & ResNet-12 & 58.5 & 76.7 & - & - \\
             MTL \cite{sun2019meta} & & ResNet-12 & 61.2 & 75.5 & - & - &  - & - \\
             vFSL \cite{variational_fsl} & & ResNet-12 & 61.2 & 77.7 & - & - & - & - \\
             Neg-cosine \cite{liu2020negative}& & ResNet-18 & 62.3 & 80.9 & - & - & 72.7 & 89.4 \\
             MetaOpt \cite{lee2019meta} & & ResNet-12 & 62.6 & 78.6 & 66.0 & 81.6 & - & -\\
             SimpleShot \cite{simpleshot} & & ResNet-18 & 62.9 & 80.0 & 68.9 & 84.6 & 68.9 & 84.0 \\
             Distill \cite{tian2020rethinking} & & ResNet-12 & 64.8 & 82.1 & 71.5 & 86.0 & - & -\\
             \midrule
             RelatNet + T \cite{can} & & ResNet-12 & 52.4 & 65.4 & - & - & - & -\\
             ProtoNet + T \cite{can} & & ResNet-12 & 55.2 & 71.1 & - & - & - & -\\
             MatchNet+T \cite{can} &  & ResNet-12 & 56.3 & 69.8 & - & - & - & -\\
             TPN \cite{liu2018learning} &  & ResNet-12 & 59.5 & 75.7 & - & - & - & -\\
             TEAM \cite{team}& & ResNet-18 & 60.1 & 75.9 & - & - & - & -\\
             Ent-min \cite{dhillon2019baseline}& & ResNet-12 & 62.4 & 74.5 & 68.4 & 83.4 & - & -\\
             CAN+T \cite{can}& & ResNet-12 & 67.2 & 80.6 & 73.2 & 84.9 & - & -\\
             LaplacianShot \cite{Laplacian}& & ResNet-18 & 72.1 & 82.3 & 79.0 & 86.4 & 81.0 & 88.7 \\
             \rowcolor{Gray} TIM-ADM & & ResNet-18 & 73.6 & \textbf{85.0} & \textbf{80.0} & \textbf{88.5} & 81.9 & 90.7 \\
             \rowcolor{Gray} TIM-GD & \multirow{-10}{*}{\cmark} & ResNet-18 & \textbf{73.9} & \textbf{85.0} & 79.9 & \textbf{88.5} & \textbf{82.2} & \textbf{90.8} \\
             \toprule
             LEO \cite{leo}& \multirow{5}{*}{\xmark} & WRN28-10 & 61.8 & 77.6 & 66.3 & 81.4 & - & -\\
             SimpleShot \cite{simpleshot}& & WRN28-10 & 63.5 & 80.3 & 69.8 & 85.3 & - & -\\
             MatchNet \cite{matching_net}& & WRN28-10 & 64.0 & 76.3 & - & - & - & -\\
             CC+rot+unlabeled \cite{gidaris2019boosting} & & WRN28-10 & 64.0 & 80.7 & 70.5 & 85.0 & - & -\\
             FEAT \cite{feat} & & WRN28-10 & 65.1 & 81.1 & 70.4 & 84.4 & - & -\\
             \midrule
             AWGIM \cite{guo2020attentive}&  & WRN28-10 & 63.1 & 78.4 & 67.7 & 82.8 & - & -\\
             Ent-min \cite{dhillon2019baseline} &  & WRN28-10 & 65.7 & 78.4 & 73.3 & 85.5 & - & -\\
             SIB  \cite{hu2020empirical} &  & WRN28-10 & 70.0 & 79.2 & - & - & - & -\\
             BD-CSPN \cite{prototype}&  & WRN28-10 & 70.3 & 81.9 & 78.7 & 86.92 & - & -\\
             LaplacianShot  \cite{Laplacian} &  & WRN28-10 & 74.9 & 84.1 & 80.2 & 87.6 & - & -\\
             \rowcolor{Gray} TIM-ADM & & WRN28-10 & 77.5 & 87.2 & 82.0 & 89.7 & - & -\\
             \rowcolor{Gray} TIM-GD & \multirow{-7}{*}{\cmark} & WRN28-10 & \textbf{77.8} & \textbf{87.4} & \textbf{82.1} & \textbf{89.8} & - & -\\
            %  \toprule
            %  SimpleShot \cite{simpleshot}& \xmark & DenseNet-121 & 64.3 & 81.5 & 71.3 & 86.7 
            %  \\
            %  \midrule
            %  LaplacianShot \cite{Laplacian}&  & DenseNet-121 & 75.6 & 84.7 & 80.3 & 87.9
            %  \\
            %  \rowcolor{Gray} TIM-ADM &  & DenseNet-121 & 76.8 & 87.3 & 83.6 & 90.6 \\
            %  \rowcolor{Gray} TIM-GD & \multirow{-3}{*}{\cmark} & DenseNet-121 & \textbf{77.4} & \textbf{88.2} & \textbf{83.7} & \textbf{90.9} \\
             \bottomrule
        \end{tabular}
        \label{tab:benchmark_results}
        \end{table}
        
        \begin{table}
            \newlength\wexp
            \settowidth{\wexp}{\textbf{\textit{mini}-ImageNet} $\rightarrow$ \textbf{CUB}}
            \centering
            \small
            \caption{The results for the domain-shift setting \textit{mini}-Imagenet $\rightarrow$ CUB. The results obtained by our models (gray-shaded) are averaged over 10,000 episodes.}
            \begin{tabular}{lcccc}
            % \begin{tabular}{lcccc*{2}{w{c}{\dimexpr.5\wexp-\tabcolsep}}}
                & & \multicolumn{1}{c}{\textbf{\textit{mini}-ImageNet} $\rightarrow$ \textbf{CUB}}\\
                 Methods & Backbone & 5-shot\\
                 \toprule
                 MatchNet \cite{matching_net} & ResNet-18 & 53.1\\
                 MAML \cite{maml} & ResNet-18 & 51.3 \\
                 ProtoNet \cite{prototypical_nets} & ResNet-18 & 62.0 \\
                 RelatNet \cite{relation_net} & ResNet-18 & 57.7 \\
                %  CL2N \cite{simpleshot} & ResNet-18 & 70.1 & 86.3 & 48.0 & 64.0 \\
                SimpleShot \cite{simpleshot} & ResNet-18 & 64.0 \\
                GNN \cite{tseng2020cross} & ResNet-10 & 66.9 \\
                Neg-Cosine \cite{liu2020negative} & ResNet-18 & 67.0 \\
                Baseline \cite{closer_look} & ResNet-18 & 65.6 \\
                LaplacianShot \cite{Laplacian} & ResNet-18 & 66.3 \\
                \rowcolor{Gray} TIM-ADM & ResNet-18 & 70.3 \\
                \rowcolor{Gray} TIM-GD & ResNet-18 & \textbf{71.0} \\
                 \bottomrule
            \end{tabular}
            \label{tab:domin_shift_results}
        \end{table}
         
    \subsection{Impact of domain-shift}   
        Chen et al. \cite{closer_look} recently showed that the performance of most meta-learning methods may drop drastically when a domain-shift exists between the base training data and test data. Surprisingly, the simplest 
        discriminative baseline exhibited the best performance in this case. Therefore, we evaluate our methods in this challenging scenario. To this end, we simulate a domain shift by training the feature encoder on \textit{mini}-Imagenet while evaluating the methods on \textit{CUB}, similarly to the setting introduced in \cite{closer_look}. TIM-GD and TIM-ADM beat previous methods by significant margins in the domain-shift scenario, consistently with our results in the standard few-shot benchmarks, thereby demonstrating an increased potential of applicability to real-world situations.

    \subsection{Pushing the meta-testing stage}
        
        Most few-shot papers only evaluate their method in the usual 5-way scenario. Nevertheless, \cite{closer_look} showed that meta-learning methods could be beaten by their discriminative baseline when more ways were introduced in each task. Therefore, we also provide results of our method in the more challenging 10-way and 20-way scenarios on \textit{mini}-ImageNet. These results, which are presented in \autoref{tab:more_ways}, show that TIM-GD outperforms other methods by significant margins, in both settings.
        \begin{table}
            \centering
            \caption{Results for increasing the number of classes on \textit{mini}-ImageNet. The results obtained by our models (gray-shaded) are averaged over 10,000 episodes.}
            \small
            \begin{tabular}{lcccccccc}
                & & \multicolumn{2}{c}{10-way} & \multicolumn{2}{c}{20-way} \\
                 Methods & Backbone & 1-shot & 5-shot & 1-shot & 5-shot\\
                 \toprule
                 MatchNet \cite{matching_net}& ResNet-18 & - & 52.3 & - & 36.8 \\
                 ProtoNet \cite{prototypical_nets}& ResNet-18 & - & 59.2 & - & 45.0 \\
                 RelatNet \cite{relation_net}& ResNet-18 & - & 53.9 & - & 39.2 \\
                 SimpleShot \cite{simpleshot}& ResNet-18 & 45.1 & 68.1 & 32.4 & 55.4 \\
                 Baseline \cite{closer_look}& ResNet-18 & - & 55.0 & - & 42.0 \\
                 Baseline++ \cite{closer_look}& ResNet-18 & - & 63.4 & - & 50.9 \\
                 \rowcolor{Gray} TIM-ADM & ResNet-18 & 56.0 & \textbf{72.9} & \textbf{39.5} & 58.8 \\
                 \rowcolor{Gray} TIM-GD & ResNet-18 & \textbf{56.1} & 72.8 & 39.3 & \textbf{59.5} \\
                 \bottomrule
            \end{tabular}
            \label{tab:more_ways}
        \end{table}

    \subsection{Ablation study}

        \textbf{Influence of each term: }\label{sec:ablation_terms} We now assess the impact of each term\footnote{The $\textbf{W}$ and $\textbf{q}$ updates of TIM-ADM associated to each configuration can be found in the supplementary material.} in our loss in Eq. (\ref{eq:tim_objective}) on the final performance of our methods. The results are reported in \autoref{tab:ablation_effect_terms}. 
        We observe that integrating the three terms in our loss consistently outperforms any other configuration. Interestingly, removing the label-marginal entropy, $\widehat{\mathcal{H}}(Y_\mathcal{Q})$, reduces significantly the performances in both TIM-GD and TIM-ADM, particularly when only classifier weights $\textbf{W}$ are 
        updated and feature extractor $\boldsymbol{\phi}$ is fixed. 
      %  (referred to as TIM-GD $\{\textbf{W}\}$ and TIM-ADM $\{\textbf{W}\}$). 
        Such a behavior could be explained by the following fact: the conditional entropy term, $\mathcal{\widehat{H}}(Y_\mathcal{Q}|X_\mathcal{Q})$, may yield degenerate solutions (assigning all query samples to a single class) on numerous tasks, when used alone. 
        % Even though the performances can be improved with careful hyperparameter tuning, as shown in supp. material,
        This emphasizes the importance of the label-marginal entropy term $\widehat{\mathcal{H}}(Y_\mathcal{Q})$ in our loss (\ref{eq:tim_objective}), which acts as a powerful regularizer to prevent such trivial solutions.
        
        \begin{table}[t]
           \small
           \centering
            \caption{Ablation study on the effect of each term in our loss in Eq. \eqref{eq:tim_objective}, when only the classifier weights are fine-tuned, i.e., updating only $\textbf{W}$, and when the whole network is fine-tuned, i.e., updating $\{\boldsymbol{\phi},\textbf{W}\}$. The results are reported for ResNet-18 as backbone. 
            The same term indexing as in Eq. \eqref{eq:tim_objective} is used here: $\widehat{\mathcal{H}}(Y_\mathcal{Q})$: Marginal entropy, $\widehat{\mathcal{H}}(Y_\mathcal{Q}|X_\mathcal{Q})$: Conditional entropy, $\mathrm{CE}$: Cross-entropy.}
           \resizebox{\textwidth}{!}{
           \begin{tabular}{ccccccccc}
                 & & & \multicolumn{2}{c}{\textbf{\textit{mini}-ImageNet}} & \multicolumn{2}{c}{\textbf{\textit{tiered}-ImageNet}} & \multicolumn{2}{c}{\textbf{CUB}}\\
                 Method & Param. & Loss & 1-shot & 5-shot & 1-shot & 5-shot & 1-shot & 5-shot \\
                 \toprule
                 \multirow{4}{*}{TIM-ADM} & \multirow{4}{*}{$\{\textbf{W}\}$} & $\mathrm{CE}$ & 60.0 & 79.6 & 68.0 & 84.6 & 68.6 & 86.4 \\
                 & & $\mathrm{CE} + \widehat{\mathcal{H}}(Y_\mathcal{Q}|X_\mathcal{Q})$ & 36.0 & 77.0 & 48.1 & 82.5 & 48.5 & 86.5 \\
                 & & $\mathrm{CE} - \widehat{\mathcal{H}}(Y_\mathcal{Q})$ & 66.7 & 82.0 & 74.0 & 86.5 & 74.2 & 88.3 \\
                 & & $\mathrm{CE} - \widehat{\mathcal{H}}(Y_\mathcal{Q}) + \widehat{\mathcal{H}}(Y_\mathcal{Q}|X_\mathcal{Q})$ & \textbf{73.6} & \textbf{85.0} & \textbf{80.0} & \textbf{88.5} & \textbf{81.9} & \textbf{90.7} \\
                 \midrule
                 \multirow{4}{*}{TIM-GD} & \multirow{4}{*}{\{$\textbf{W} $\}}& $\mathrm{CE}$ & 60.7 & 79.4 & 68.4 & 84.3 & 69.6 & 86.3 \\
                 & & $\mathrm{CE} + \widehat{\mathcal{H}}(Y_\mathcal{Q}|X_\mathcal{Q})$ & 35.3 & 79.2 & 45.9 & 80.6 & 46.1 & 85.9 \\
                 & & $\mathrm{CE} - \widehat{\mathcal{H}}(Y_\mathcal{Q})$ & 66.1 & 81.3 & 73.4 & 86.0 & 73.9 & 88.0 \\
                 & & $\mathrm{CE} - \widehat{\mathcal{H}}(Y_\mathcal{Q}) + \widehat{\mathcal{H}}(Y_\mathcal{Q}|X_\mathcal{Q})$ & \textbf{73.9} & \textbf{85.0} & \textbf{79.9} & \textbf{88.5} & \textbf{82.2} & \textbf{90.8} \\
                 \midrule
                 \multirow{4}{*}{TIM-GD} & \multirow{4}{*}{$\{\boldsymbol{\phi}, \textbf{W}\}$}& $\mathrm{CE}$ & 60.8 & 81.6 & 65.7 & 83.5 & 68.7 & 87.7\\
                 & & $\mathrm{CE} + \widehat{\mathcal{H}}(Y_\mathcal{Q}|X_\mathcal{Q})$ & 62.7 & 81.9 & 66.9 & 82.8 & 72.6 & 89.0 \\
                 & & $\mathrm{CE} - \widehat{\mathcal{H}}(Y_\mathcal{Q})$ & 62.3 & 82.7 & 68.3 & 85.4 & 70.7 & 88.8 \\
                %  & & $\mathrm{CE} - \widehat{\mathcal{H}}(Y) + \widehat{\mathcal{H}}(Y|X)$ & 67.2 & 83.9 & 73.1 & 86.6 & 76.4 & 89.9 \\
                 & & $\mathrm{CE} - \widehat{\mathcal{H}}(Y_\mathcal{Q}) + \widehat{\mathcal{H}}(Y_\mathcal{Q}|X_\mathcal{Q})$ & \textbf{67.2} & \textbf{84.7} & \textbf{73.0} & \textbf{86.8} & \textbf{76.7} & \textbf{90.5} \\
                 \bottomrule
            \end{tabular}}
            \label{tab:ablation_effect_terms}
        \end{table}


        \textbf{Fine-tuning the whole network vs only the classifier weights: }
            While our TIM-GD and TIM-ADM optimize w.r.t $\textbf{W}$ and keep base-trained encoder $f_{\boldsymbol{\phi}}$ fixed at inference, the authors of \cite{dhillon2019baseline} fine-tuned the whole network $\{\textbf{W}, \boldsymbol{\phi}\}$ when performing their transductive entropy minimization. To assess both approaches, we add to \autoref{tab:ablation_effect_terms} a variant of TIM-GD, in which we fine-tune the whole network $\{\textbf{W}, \boldsymbol{\phi}\}$, by using the same optimization procedure as in \cite{dhillon2019baseline}. We found that, besides being much slower, fine-tuning the whole network for our objective in Eq. \ref{eq:tim_objective} degrades the performances, as also conveyed by the convergence plots in \autoref{fig:convergence_methods}. 
            %Such results validate our initial optimization choice. 
            Interestingly, when fine-tuning the whole network $\{\textbf{W}, \boldsymbol{\phi}\}$,  the absence of $\widehat{\mathcal{H}}(Y_\mathcal{Q})$ in the entropy-based loss $\mathrm{CE} + \widehat{\mathcal{H}}(Y_\mathcal{Q}|X_\mathcal{Q})$ does not cause the same drastic drop in performance as observed earlier when optimizing with respect to $\textbf{W}$ only. We hypothesize that the network's intrinsic regularization (such as batch normalizations) and the use of small learning rates, as prescribed by \cite{dhillon2019baseline}, help the optimization process, preventing the predictions from approaching the vertices of the simplex, where entropy's gradients diverge.

        % \textbf{Influence of the prior:}  In standard few-shot benchmarks, the tasks are balanced, i.e., the class-distribution prior is uniform. However, support-based prior proves its superiority under a non-uniform distribution scenario. Specifically, we evaluated our method on iNat, a recently introduced benchmark \cite{inat_benchmark} with severe imbalance across classes, as depicted on \autoref{fig:inat_distrib}. For this large task, TIM-GD is ran for 1000 epochs (instead of 150 in all other experiments). Table \ref{tab:ablation_effect_prior} reports the results, including both when a uniform prior is assumed and when the prior is derived from the empirical ground truth marginal distribution on the support set $\mathcal{S}$, as in Eq. \eqref{eq:tim_objective}. Integrating a support-based prior yields an approximate $5 \%$ of relative improvement, hence confirming the strong regularizing effect of leveraging support-based label statistics.

        % \begin{table}
        %     \centering
        %     \begin{tabular}{ccccc}
        %          &  \multicolumn{3}{c}{\textbf{Meta-iNat}} \\
        %          \toprule
        %          Method & Conv4 & ResNet18 & WRN \\
        %          \toprule
        %          L2N \cite{simpleshot}& 23.7 & 58.5 & 63.8 \\
        %          \rowcolor{Gray} TIM-GD & 22.2 & 59.0 & 65.0 \\
        %          \rowcolor{Gray} TGIM-GD & \textbf{27.0} & \textbf{63.8} & \textbf{69.0} \\
        %          \bottomrule
        %     \end{tabular}
        %     \caption{Ablation study. Importance of the accuracy of prior class distribution on a highly unbalanced task. TIM-GD implicitly assumes a prior distribution over labels, while TGIM-GD encourages query distribution to respect the same distribution as the one on support.}
        %     \label{tab:ablation_effect_prior}
        % \end{table}


    \subsection{Inference run-times}
        Transductive methods are generally slower at inference than their inductive counterparts, with run-times that are, typically, several orders of magnitude larger. In \autoref{tab:runtimes}, we measure the average adaptation time per few-shot task, defined as the time required by each method to build the final classifier, for a 5-shot 5-way task on \textit{mini}-ImageNet using the WRN28-10 network. Table \ref{tab:runtimes} conveys that our ADM optimization gains one order of magnitude in run-time over our gradient-based method, and more than two orders of magnitude in comparison to \cite{dhillon2019baseline}, which fine-tunes the whole network. Note that TIM-ADM still remains slower than the inductive baseline. Our methods were run on the same GTX 1080 Ti GPU, while the run-time of \cite{dhillon2019baseline} is directly reported from the paper. 

        % \begin{figure}
        %     \CenterFloatBoxes
        %     \begin{floatrow}
        %         \ffigbox[\FBwidth]{
        %             \includegraphics[scale=0.35]{figures/iNat_class_distrib.pdf}
        %         }{\vspace{-1em}
        %         \caption{Heavy-tailed class distribution on the 227-way task of Meta-iNat.}
        %         \label{fig:inat_distrib}
        %         }
        %         \killfloatstyle
        %         \capbtabbox[\FBwidth]{
        %             \caption{Importance of the prior class distribution on the Meta-iNat highly imbalanced task. To the best of our knowledge, the L2N method from \cite{simpleshot} represents the state-of-the-art on this task.}
        %             }{\small
        %              \begin{tabular}{cccc}
        %                 \multicolumn{4}{c}{\textbf{Meta-iNat}} \\
        %                 \toprule
        %                 Method & Prior & ResNet-18 & WRN \\
        %                 \toprule
        %                 %  UN \cite{simpleshot}& - & 58.1 & 63.2 \\
        %                 SimpleShot \cite{simpleshot}& - & 58.5 & 63.8 \\
        %                 \rowcolor{Gray}  & Uniform & - & - \\
        %                 \rowcolor{Gray} \multirow{-2}{*}{TIM-ADM}& $\mathcal{S}$-based & \textbf{64.7} & \textbf{71.1} \\
        %                 \rowcolor{Gray}  & Uniform & - & - \\
        %                 \rowcolor{Gray} \multirow{-2}{*}{TIM-GD}& $\mathcal{S}$-based & 64.3 & 70.9 \\
        %                 \bottomrule
        %             \end{tabular}
        %             \label{tab:ablation_effect_prior}
        %             }%
        %     \end{floatrow}
        % \end{figure}
    
        % \begin{figure}
        %     \CenterFloatBoxes
        %     \begin{floatrow}
        %     \ffigbox[\FBwidth]{
        %       \includegraphics[scale=0.30]{figures/runtimes/mini.pdf}
        %     }{
        %     \vspace{-1em}
        %       \caption{Convergence plots for our methods on \textit{mini}-ImageNet with a ResNet-18. Solid lines are averages, while shadows are 95\% confidence intervals. Time is in logarithmic scale.}
        %       \label{fig:convergence_methods}
        %     }
        %     \killfloatstyle
        %     \capbtabbox{
        %         \small
        %         \begin{tabular}{lcc}
        %             \multicolumn{3}{c}{\textbf{Runtimes}} \\
        %             \toprule
        %             Method & Param. & Infer./task (s) \\
        %             \toprule
        %             Simp.Shot \cite{simpleshot}& $\{\textbf{W}\}$ &  9.0 $e^{-3}$ \\
        %             % \midrule
        %             Lapl.Shot \cite{Laplacian}$^{\dagger}$ & $\{\textbf{W}\}$ & 1.2 $e^{-2}$ \\
        %             \rowcolor{Gray} TIM-ADM $^{\dagger}$ & $\{\textbf{W}\}$ & 1.2 $e^{-1}$\\
        %             \rowcolor{Gray} TIM-GD $^{\dagger}$ & $\{\textbf{W}\}$ & 2.2 $e^{+0}$\\
        %             Ent-min $^{\ddagger}$ \cite{dhillon2019baseline} & $\{\boldsymbol{\phi}, \textbf{W}\}$ & 2.1 $ e^{+1}$ \\
        %             \bottomrule
        %         \end{tabular}
        %     }{
        %       \caption{Inference runtime per task for a 5-shot 5-way task on mini-ImageNet with a WRN28-10 backbone. Methods marked with $^{\dagger}$ are transductive.}%
        %       \label{tab:runtimes}
        %     }
        %     \end{floatrow}
        % \end{figure}
        \begin{figure}[t]
            \centering
            \includegraphics[scale=0.4]{figures/runtimes/mini.pdf}
            \caption{Convergence plots for our methods on \textit{mini}-ImageNet with a ResNet-18. Solid lines are averages, while shadows are 95\% confidence intervals. Time is in logarithmic scale. \textbf{Left:} Evolution of the test accuracy during transductive inference. \textbf{Right:} Evolution of the mutual information between query features and predictions $\widehat{\mathcal{I}}(X_\mathcal{Q};Y_\mathcal{Q})$, computed as in Eq. (\ref{prior-aware-MI}), with $\alpha=1$.}
            \label{fig:convergence_methods}
        \end{figure}
        
        \begin{table}[t]
            \centering
                \begin{tabular}{lccc}
                    \multicolumn{4}{c}{\textbf{Run-times}} \\
                    \toprule
                    Method & Parameters & Transductive & Inference/task (s) \\
                    \toprule
                    SimpleShot \cite{simpleshot}& $\{\textbf{W}\}$ & \xmark & $9.0 \times 10^{-3}$ \\
                    \midrule
                    % LaplacianShot & $\{\textbf{W}\}$ & & $1.2 \times 10^{-2}$ \\
                    \rowcolor{Gray} TIM-ADM & $\{\textbf{W}\}$ & & $1.2 \times 10^{-1}$\\
                    \rowcolor{Gray} TIM-GD & $\{\textbf{W}\}$ & & $2.2 \times 10^{+0}$\\
                    Ent-min \cite{dhillon2019baseline} & $\{\boldsymbol{\phi}, \textbf{W}\}$ & \multirow{-4}{*}{\cmark} & $2.1 \times 10^{+1}$ \\
                    \bottomrule
                \end{tabular}
            \caption{Inference run-time per few-shot task for a 5-shot 5-way task on mini-ImageNet with a WRN28-10 backbone.}
            \label{tab:runtimes}
        \end{table}



==> Neurips 2021 (4)/3_experiments.tex <==
\section{Experiments}

    \textbf{Hyperparameters: } To keep our experiments as simple as possible, \textbf{our hyperparameters are kept fixed across all the experiments and methods (TIM-GD and TIM-ADM)}. The conditional entropy weight $\alpha$ and the cross-entropy weights $\lambda$ in Objective (\ref{eq:tim_objective}) are both set to $0.1$. The temperature parameter $\tau$ in the classifier is set to 15. 
    % In supp. material, however, we show that tuning $\tau$ and $\lambda$ on the validation set can further improve the performance. 
    In our TIM-GD method, we use the ADAM optimizer with the recommended parameters \cite{kingma2014adam}, and run 1000 iterations for each task. For TIM-ADM, we run 150 iterations.
    
    \textbf{Base-training procedure:} The feature extractors are trained following the same simple base-training procedure as in \cite{Laplacian} and using standard networks (ResNet-18 and WRN28-10), for all the experiments. Specifically, they are trained using the standard cross-entropy loss on the base classes, with label smoothing. The label-smoothing parameter is set to 0.1. We emphasize that base training does not involve any meta-learning or episodic training strategy. The models are trained for 90 epochs, with the learning rate initialized to 0.1, and divided by 10 at epochs 45 and 66. Batch size is set to 256 for ResNet-18, and to 128 for WRN28-10. During training, all the images are resized to $84 \times 84$, and we used the same data augmentation procedure as in \cite{Laplacian}, which includes random cropping, color jitter  and random horizontal flipping. 

    \textbf{Datasets: } We resort to 3 few-shot learning  datasets to benchmark the proposed models. As standard few-shot benchmarks, we use the \textbf{\textit{mini}-Imagenet} \cite{matching_net} dataset, with 100 classes split as in \cite{ravi2016optimization}, the \textbf{Caltech-UCSD Birds 200} \cite{cub} (CUB) dataset, with 200 classes, split following \cite{closer_look}, and finally the larger \textbf{\textit{tiered}-Imagenet} dataset, with 608 classes split as in \cite{tiered_imagenet}.
    % Finally, we used the challenging and more realistic \textbf{meta-iNat} dataset \cite{inat}, with 908 classes and severe class imbalance, split according to \cite{inat_benchmark}.

    \subsection{Comparison to state-of-the-art}\label{sec:benchmark}

        We first evaluate our methods TIM-GD and TIM-ADM on the widely adopted \textit{mini}-ImageNet, \textit{tiered}-ImageNet and \textit{CUB} benchmark datasets, in the most common 1-shot 5-way and 5-shot 5-way scenarios, with 15 query shots for each class. Results are reported in \autoref{tab:benchmark_results}, and are averaged over 10,000 episodes, following \cite{simpleshot}. We can observe that both TIM-GD and TIM-ADM yield state-of-the-art performances, consistently across all standard datasets, scenarios and backbones, improving over both transductive and inductive methods, by significant margins. 
        % In supp. material, we further show the superiority of our methods in the 10 and 20-way s
        %and outperforming the best performing methods by over $5\%$ in the 1-shot setting.
        %and $4\%$ on 5-shot tasks.
        
        \begin{table}
        \centering
        \small
        \caption{Comparison to the state-of-the-art methods on \textit{mini}-ImageNet, \textit{tiered}-Imagenet and CUB. The methods are sub-grouped into transductive and inductive methods, as well as by backbone architecture. Our results (gray-shaded) are averaged over 10,000 episodes. "-" signifies the result is unavailable.}
        \begin{tabular}{lccccccccc}
            & & &\multicolumn{2}{c}{\textbf{\textit{mini}-ImageNet}} & \multicolumn{2}{c}{\textbf{\textit{tiered}-ImageNet}} & \multicolumn{2}{c}{\textbf{CUB}} \\
             Method & Transd. & Backbone & 1-shot & 5-shot & 1-shot & 5-shot & 1-shot & 5-shot\\
             \toprule
             MAML \cite{maml}& \multirow{9}{*}{\xmark} & ResNet-18 & 49.6 & 65.7 & - & - & 68.4 & 83.5 \\
            %  Baseline++ \cite{closer_look}& & ResNet-18 & 51.9 & 75.7 & - & - \\
             RelatNet \cite{relation_net}& & ResNet-18 & 52.5 & 69.8 &  - & - & 68.6 & 84.0 \\
             MatchNet \cite{matching_net}& & ResNet-18 & 52.9 & 68.9 &  - & - & 73.5 & 84.5 \\
             ProtoNet \cite{prototypical_nets}& & ResNet-18 & 54.2 & 73.4 &  - & - & 73.0 & 86.6 \\
            %  TADAM \cite{tadam} & & ResNet-12 & 58.5 & 76.7 & - & - \\
             MTL \cite{sun2019meta} & & ResNet-12 & 61.2 & 75.5 & - & - &  - & - \\
             vFSL \cite{variational_fsl} & & ResNet-12 & 61.2 & 77.7 & - & - & - & - \\
             Neg-cosine \cite{liu2020negative}& & ResNet-18 & 62.3 & 80.9 & - & - & 72.7 & 89.4 \\
             MetaOpt \cite{lee2019meta} & & ResNet-12 & 62.6 & 78.6 & 66.0 & 81.6 & - & -\\
             SimpleShot \cite{simpleshot} & & ResNet-18 & 62.9 & 80.0 & 68.9 & 84.6 & 68.9 & 84.0 \\
             Distill \cite{tian2020rethinking} & & ResNet-12 & 64.8 & 82.1 & 71.5 & 86.0 & - & -\\
             \midrule
             RelatNet + T \cite{can} & & ResNet-12 & 52.4 & 65.4 & - & - & - & -\\
             ProtoNet + T \cite{can} & & ResNet-12 & 55.2 & 71.1 & - & - & - & -\\
             MatchNet+T \cite{can} &  & ResNet-12 & 56.3 & 69.8 & - & - & - & -\\
             TPN \cite{liu2018learning} &  & ResNet-12 & 59.5 & 75.7 & - & - & - & -\\
             TEAM \cite{team}& & ResNet-18 & 60.1 & 75.9 & - & - & - & -\\
             Ent-min \cite{dhillon2019baseline}& & ResNet-12 & 62.4 & 74.5 & 68.4 & 83.4 & - & -\\
             CAN+T \cite{can}& & ResNet-12 & 67.2 & 80.6 & 73.2 & 84.9 & - & -\\
             LaplacianShot \cite{Laplacian}& & ResNet-18 & 72.1 & 82.3 & 79.0 & 86.4 & 81.0 & 88.7 \\
             \rowcolor{Gray} TIM-ADM & & ResNet-18 & 73.6 & \textbf{85.0} & \textbf{80.0} & \textbf{88.5} & 81.9 & 90.7 \\
             \rowcolor{Gray} TIM-GD & \multirow{-10}{*}{\cmark} & ResNet-18 & \textbf{73.9} & \textbf{85.0} & 79.9 & \textbf{88.5} & \textbf{82.2} & \textbf{90.8} \\
             \toprule
             LEO \cite{leo}& \multirow{5}{*}{\xmark} & WRN28-10 & 61.8 & 77.6 & 66.3 & 81.4 & - & -\\
             SimpleShot \cite{simpleshot}& & WRN28-10 & 63.5 & 80.3 & 69.8 & 85.3 & - & -\\
             MatchNet \cite{matching_net}& & WRN28-10 & 64.0 & 76.3 & - & - & - & -\\
             CC+rot+unlabeled \cite{gidaris2019boosting} & & WRN28-10 & 64.0 & 80.7 & 70.5 & 85.0 & - & -\\
             FEAT \cite{feat} & & WRN28-10 & 65.1 & 81.1 & 70.4 & 84.4 & - & -\\
             \midrule
             AWGIM \cite{guo2020attentive}&  & WRN28-10 & 63.1 & 78.4 & 67.7 & 82.8 & - & -\\
             Ent-min \cite{dhillon2019baseline} &  & WRN28-10 & 65.7 & 78.4 & 73.3 & 85.5 & - & -\\
             SIB  \cite{hu2020empirical} &  & WRN28-10 & 70.0 & 79.2 & - & - & - & -\\
             BD-CSPN \cite{prototype}&  & WRN28-10 & 70.3 & 81.9 & 78.7 & 86.92 & - & -\\
             LaplacianShot  \cite{Laplacian} &  & WRN28-10 & 74.9 & 84.1 & 80.2 & 87.6 & - & -\\
             \rowcolor{Gray} TIM-ADM & & WRN28-10 & 77.5 & 87.2 & 82.0 & 89.7 & - & -\\
             \rowcolor{Gray} TIM-GD & \multirow{-7}{*}{\cmark} & WRN28-10 & \textbf{77.8} & \textbf{87.4} & \textbf{82.1} & \textbf{89.8} & - & -\\
            %  \toprule
            %  SimpleShot \cite{simpleshot}& \xmark & DenseNet-121 & 64.3 & 81.5 & 71.3 & 86.7 
            %  \\
            %  \midrule
            %  LaplacianShot \cite{Laplacian}&  & DenseNet-121 & 75.6 & 84.7 & 80.3 & 87.9
            %  \\
            %  \rowcolor{Gray} TIM-ADM &  & DenseNet-121 & 76.8 & 87.3 & 83.6 & 90.6 \\
            %  \rowcolor{Gray} TIM-GD & \multirow{-3}{*}{\cmark} & DenseNet-121 & \textbf{77.4} & \textbf{88.2} & \textbf{83.7} & \textbf{90.9} \\
             \bottomrule
        \end{tabular}
        \label{tab:benchmark_results}
        \end{table}
        
        \begin{table}
            \newlength\wexp
            \settowidth{\wexp}{\textbf{\textit{mini}-ImageNet} $\rightarrow$ \textbf{CUB}}
            \centering
            \small
            \caption{The results for the domain-shift setting \textit{mini}-Imagenet $\rightarrow$ CUB. The results obtained by our models (gray-shaded) are averaged over 10,000 episodes.}
            \begin{tabular}{lcccc}
            % \begin{tabular}{lcccc*{2}{w{c}{\dimexpr.5\wexp-\tabcolsep}}}
                & & \multicolumn{1}{c}{\textbf{\textit{mini}-ImageNet} $\rightarrow$ \textbf{CUB}}\\
                 Methods & Backbone & 5-shot\\
                 \toprule
                 MatchNet \cite{matching_net} & ResNet-18 & 53.1\\
                 MAML \cite{maml} & ResNet-18 & 51.3 \\
                 ProtoNet \cite{prototypical_nets} & ResNet-18 & 62.0 \\
                 RelatNet \cite{relation_net} & ResNet-18 & 57.7 \\
                %  CL2N \cite{simpleshot} & ResNet-18 & 70.1 & 86.3 & 48.0 & 64.0 \\
                SimpleShot \cite{simpleshot} & ResNet-18 & 64.0 \\
                GNN \cite{tseng2020cross} & ResNet-10 & 66.9 \\
                Neg-Cosine \cite{liu2020negative} & ResNet-18 & 67.0 \\
                Baseline \cite{closer_look} & ResNet-18 & 65.6 \\
                LaplacianShot \cite{Laplacian} & ResNet-18 & 66.3 \\
                \rowcolor{Gray} TIM-ADM & ResNet-18 & 70.3 \\
                \rowcolor{Gray} TIM-GD & ResNet-18 & \textbf{71.0} \\
                 \bottomrule
            \end{tabular}
            \label{tab:domin_shift_results}
        \end{table}
         
    \subsection{Impact of domain-shift}   
        Chen et al. \cite{closer_look} recently showed that the performance of most meta-learning methods may drop drastically when a domain-shift exists between the base training data and test data. Surprisingly, the simplest 
        discriminative baseline exhibited the best performance in this case. Therefore, we evaluate our methods in this challenging scenario. To this end, we simulate a domain shift by training the feature encoder on \textit{mini}-Imagenet while evaluating the methods on \textit{CUB}, similarly to the setting introduced in \cite{closer_look}. TIM-GD and TIM-ADM beat previous methods by significant margins in the domain-shift scenario, consistently with our results in the standard few-shot benchmarks, thereby demonstrating an increased potential of applicability to real-world situations.

    \subsection{Pushing the meta-testing stage}
        
        Most few-shot papers only evaluate their method in the usual 5-way scenario. Nevertheless, \cite{closer_look} showed that meta-learning methods could be beaten by their discriminative baseline when more ways were introduced in each task. Therefore, we also provide results of our method in the more challenging 10-way and 20-way scenarios on \textit{mini}-ImageNet. These results, which are presented in \autoref{tab:more_ways}, show that TIM-GD outperforms other methods by significant margins, in both settings.
        \begin{table}
            \centering
            \caption{Results for increasing the number of classes on \textit{mini}-ImageNet. The results obtained by our models (gray-shaded) are averaged over 10,000 episodes.}
            \small
            \begin{tabular}{lcccccccc}
                & & \multicolumn{2}{c}{10-way} & \multicolumn{2}{c}{20-way} \\
                 Methods & Backbone & 1-shot & 5-shot & 1-shot & 5-shot\\
                 \toprule
                 MatchNet \cite{matching_net}& ResNet-18 & - & 52.3 & - & 36.8 \\
                 ProtoNet \cite{prototypical_nets}& ResNet-18 & - & 59.2 & - & 45.0 \\
                 RelatNet \cite{relation_net}& ResNet-18 & - & 53.9 & - & 39.2 \\
                 SimpleShot \cite{simpleshot}& ResNet-18 & 45.1 & 68.1 & 32.4 & 55.4 \\
                 Baseline \cite{closer_look}& ResNet-18 & - & 55.0 & - & 42.0 \\
                 Baseline++ \cite{closer_look}& ResNet-18 & - & 63.4 & - & 50.9 \\
                 \rowcolor{Gray} TIM-ADM & ResNet-18 & 56.0 & \textbf{72.9} & \textbf{39.5} & 58.8 \\
                 \rowcolor{Gray} TIM-GD & ResNet-18 & \textbf{56.1} & 72.8 & 39.3 & \textbf{59.5} \\
                 \bottomrule
            \end{tabular}
            \label{tab:more_ways}
        \end{table}

    \subsection{Ablation study}

        \textbf{Influence of each term: }\label{sec:ablation_terms} We now assess the impact of each term\footnote{The $\textbf{W}$ and $\textbf{q}$ updates of TIM-ADM associated to each configuration can be found in the supplementary material.} in our loss in Eq. (\ref{eq:tim_objective}) on the final performance of our methods. The results are reported in \autoref{tab:ablation_effect_terms}. 
        We observe that integrating the three terms in our loss consistently outperforms any other configuration. Interestingly, removing the label-marginal entropy, $\widehat{\mathcal{H}}(Y_\mathcal{Q})$, reduces significantly the performances in both TIM-GD and TIM-ADM, particularly when only classifier weights $\textbf{W}$ are 
        updated and feature extractor $\boldsymbol{\phi}$ is fixed. 
      %  (referred to as TIM-GD $\{\textbf{W}\}$ and TIM-ADM $\{\textbf{W}\}$). 
        Such a behavior could be explained by the following fact: the conditional entropy term, $\mathcal{\widehat{H}}(Y_\mathcal{Q}|X_\mathcal{Q})$, may yield degenerate solutions (assigning all query samples to a single class) on numerous tasks, when used alone. 
        % Even though the performances can be improved with careful hyperparameter tuning, as shown in supp. material,
        This emphasizes the importance of the label-marginal entropy term $\widehat{\mathcal{H}}(Y_\mathcal{Q})$ in our loss (\ref{eq:tim_objective}), which acts as a powerful regularizer to prevent such trivial solutions.
        
        \begin{table}[t]
           \small
           \centering
            \caption{Ablation study on the effect of each term in our loss in Eq. \eqref{eq:tim_objective}, when only the classifier weights are fine-tuned, i.e., updating only $\textbf{W}$, and when the whole network is fine-tuned, i.e., updating $\{\boldsymbol{\phi},\textbf{W}\}$. The results are reported for ResNet-18 as backbone. 
            The same term indexing as in Eq. \eqref{eq:tim_objective} is used here: $\widehat{\mathcal{H}}(Y_\mathcal{Q})$: Marginal entropy, $\widehat{\mathcal{H}}(Y_\mathcal{Q}|X_\mathcal{Q})$: Conditional entropy, $\mathrm{CE}$: Cross-entropy.}
           \resizebox{\textwidth}{!}{
           \begin{tabular}{ccccccccc}
                 & & & \multicolumn{2}{c}{\textbf{\textit{mini}-ImageNet}} & \multicolumn{2}{c}{\textbf{\textit{tiered}-ImageNet}} & \multicolumn{2}{c}{\textbf{CUB}}\\
                 Method & Param. & Loss & 1-shot & 5-shot & 1-shot & 5-shot & 1-shot & 5-shot \\
                 \toprule
                 \multirow{4}{*}{TIM-ADM} & \multirow{4}{*}{$\{\textbf{W}\}$} & $\mathrm{CE}$ & 60.0 & 79.6 & 68.0 & 84.6 & 68.6 & 86.4 \\
                 & & $\mathrm{CE} + \widehat{\mathcal{H}}(Y_\mathcal{Q}|X_\mathcal{Q})$ & 36.0 & 77.0 & 48.1 & 82.5 & 48.5 & 86.5 \\
                 & & $\mathrm{CE} - \widehat{\mathcal{H}}(Y_\mathcal{Q})$ & 66.7 & 82.0 & 74.0 & 86.5 & 74.2 & 88.3 \\
                 & & $\mathrm{CE} - \widehat{\mathcal{H}}(Y_\mathcal{Q}) + \widehat{\mathcal{H}}(Y_\mathcal{Q}|X_\mathcal{Q})$ & \textbf{73.6} & \textbf{85.0} & \textbf{80.0} & \textbf{88.5} & \textbf{81.9} & \textbf{90.7} \\
                 \midrule
                 \multirow{4}{*}{TIM-GD} & \multirow{4}{*}{\{$\textbf{W} $\}}& $\mathrm{CE}$ & 60.7 & 79.4 & 68.4 & 84.3 & 69.6 & 86.3 \\
                 & & $\mathrm{CE} + \widehat{\mathcal{H}}(Y_\mathcal{Q}|X_\mathcal{Q})$ & 35.3 & 79.2 & 45.9 & 80.6 & 46.1 & 85.9 \\
                 & & $\mathrm{CE} - \widehat{\mathcal{H}}(Y_\mathcal{Q})$ & 66.1 & 81.3 & 73.4 & 86.0 & 73.9 & 88.0 \\
                 & & $\mathrm{CE} - \widehat{\mathcal{H}}(Y_\mathcal{Q}) + \widehat{\mathcal{H}}(Y_\mathcal{Q}|X_\mathcal{Q})$ & \textbf{73.9} & \textbf{85.0} & \textbf{79.9} & \textbf{88.5} & \textbf{82.2} & \textbf{90.8} \\
                 \midrule
                 \multirow{4}{*}{TIM-GD} & \multirow{4}{*}{$\{\boldsymbol{\phi}, \textbf{W}\}$}& $\mathrm{CE}$ & 60.8 & 81.6 & 65.7 & 83.5 & 68.7 & 87.7\\
                 & & $\mathrm{CE} + \widehat{\mathcal{H}}(Y_\mathcal{Q}|X_\mathcal{Q})$ & 62.7 & 81.9 & 66.9 & 82.8 & 72.6 & 89.0 \\
                 & & $\mathrm{CE} - \widehat{\mathcal{H}}(Y_\mathcal{Q})$ & 62.3 & 82.7 & 68.3 & 85.4 & 70.7 & 88.8 \\
                %  & & $\mathrm{CE} - \widehat{\mathcal{H}}(Y) + \widehat{\mathcal{H}}(Y|X)$ & 67.2 & 83.9 & 73.1 & 86.6 & 76.4 & 89.9 \\
                 & & $\mathrm{CE} - \widehat{\mathcal{H}}(Y_\mathcal{Q}) + \widehat{\mathcal{H}}(Y_\mathcal{Q}|X_\mathcal{Q})$ & \textbf{67.2} & \textbf{84.7} & \textbf{73.0} & \textbf{86.8} & \textbf{76.7} & \textbf{90.5} \\
                 \bottomrule
            \end{tabular}}
            \label{tab:ablation_effect_terms}
        \end{table}


        \textbf{Fine-tuning the whole network vs only the classifier weights: }
            While our TIM-GD and TIM-ADM optimize w.r.t $\textbf{W}$ and keep base-trained encoder $f_{\boldsymbol{\phi}}$ fixed at inference, the authors of \cite{dhillon2019baseline} fine-tuned the whole network $\{\textbf{W}, \boldsymbol{\phi}\}$ when performing their transductive entropy minimization. To assess both approaches, we add to \autoref{tab:ablation_effect_terms} a variant of TIM-GD, in which we fine-tune the whole network $\{\textbf{W}, \boldsymbol{\phi}\}$, by using the same optimization procedure as in \cite{dhillon2019baseline}. We found that, besides being much slower, fine-tuning the whole network for our objective in Eq. \ref{eq:tim_objective} degrades the performances, as also conveyed by the convergence plots in \autoref{fig:convergence_methods}. 
            %Such results validate our initial optimization choice. 
            Interestingly, when fine-tuning the whole network $\{\textbf{W}, \boldsymbol{\phi}\}$,  the absence of $\widehat{\mathcal{H}}(Y_\mathcal{Q})$ in the entropy-based loss $\mathrm{CE} + \widehat{\mathcal{H}}(Y_\mathcal{Q}|X_\mathcal{Q})$ does not cause the same drastic drop in performance as observed earlier when optimizing with respect to $\textbf{W}$ only. We hypothesize that the network's intrinsic regularization (such as batch normalizations) and the use of small learning rates, as prescribed by \cite{dhillon2019baseline}, help the optimization process, preventing the predictions from approaching the vertices of the simplex, where entropy's gradients diverge.

        % \textbf{Influence of the prior:}  In standard few-shot benchmarks, the tasks are balanced, i.e., the class-distribution prior is uniform. However, support-based prior proves its superiority under a non-uniform distribution scenario. Specifically, we evaluated our method on iNat, a recently introduced benchmark \cite{inat_benchmark} with severe imbalance across classes, as depicted on \autoref{fig:inat_distrib}. For this large task, TIM-GD is ran for 1000 epochs (instead of 150 in all other experiments). Table \ref{tab:ablation_effect_prior} reports the results, including both when a uniform prior is assumed and when the prior is derived from the empirical ground truth marginal distribution on the support set $\mathcal{S}$, as in Eq. \eqref{eq:tim_objective}. Integrating a support-based prior yields an approximate $5 \%$ of relative improvement, hence confirming the strong regularizing effect of leveraging support-based label statistics.

        % \begin{table}
        %     \centering
        %     \begin{tabular}{ccccc}
        %          &  \multicolumn{3}{c}{\textbf{Meta-iNat}} \\
        %          \toprule
        %          Method & Conv4 & ResNet18 & WRN \\
        %          \toprule
        %          L2N \cite{simpleshot}& 23.7 & 58.5 & 63.8 \\
        %          \rowcolor{Gray} TIM-GD & 22.2 & 59.0 & 65.0 \\
        %          \rowcolor{Gray} TGIM-GD & \textbf{27.0} & \textbf{63.8} & \textbf{69.0} \\
        %          \bottomrule
        %     \end{tabular}
        %     \caption{Ablation study. Importance of the accuracy of prior class distribution on a highly unbalanced task. TIM-GD implicitly assumes a prior distribution over labels, while TGIM-GD encourages query distribution to respect the same distribution as the one on support.}
        %     \label{tab:ablation_effect_prior}
        % \end{table}


    \subsection{Inference run-times}
        Transductive methods are generally slower at inference than their inductive counterparts, with run-times that are, typically, several orders of magnitude larger. In \autoref{tab:runtimes}, we measure the average adaptation time per few-shot task, defined as the time required by each method to build the final classifier, for a 5-shot 5-way task on \textit{mini}-ImageNet using the WRN28-10 network. Table \ref{tab:runtimes} conveys that our ADM optimization gains one order of magnitude in run-time over our gradient-based method, and more than two orders of magnitude in comparison to \cite{dhillon2019baseline}, which fine-tunes the whole network. Note that TIM-ADM still remains slower than the inductive baseline. Our methods were run on the same GTX 1080 Ti GPU, while the run-time of \cite{dhillon2019baseline} is directly reported from the paper. 

        % \begin{figure}
        %     \CenterFloatBoxes
        %     \begin{floatrow}
        %         \ffigbox[\FBwidth]{
        %             \includegraphics[scale=0.35]{figures/iNat_class_distrib.pdf}
        %         }{\vspace{-1em}
        %         \caption{Heavy-tailed class distribution on the 227-way task of Meta-iNat.}
        %         \label{fig:inat_distrib}
        %         }
        %         \killfloatstyle
        %         \capbtabbox[\FBwidth]{
        %             \caption{Importance of the prior class distribution on the Meta-iNat highly imbalanced task. To the best of our knowledge, the L2N method from \cite{simpleshot} represents the state-of-the-art on this task.}
        %             }{\small
        %              \begin{tabular}{cccc}
        %                 \multicolumn{4}{c}{\textbf{Meta-iNat}} \\
        %                 \toprule
        %                 Method & Prior & ResNet-18 & WRN \\
        %                 \toprule
        %                 %  UN \cite{simpleshot}& - & 58.1 & 63.2 \\
        %                 SimpleShot \cite{simpleshot}& - & 58.5 & 63.8 \\
        %                 \rowcolor{Gray}  & Uniform & - & - \\
        %                 \rowcolor{Gray} \multirow{-2}{*}{TIM-ADM}& $\mathcal{S}$-based & \textbf{64.7} & \textbf{71.1} \\
        %                 \rowcolor{Gray}  & Uniform & - & - \\
        %                 \rowcolor{Gray} \multirow{-2}{*}{TIM-GD}& $\mathcal{S}$-based & 64.3 & 70.9 \\
        %                 \bottomrule
        %             \end{tabular}
        %             \label{tab:ablation_effect_prior}
        %             }%
        %     \end{floatrow}
        % \end{figure}
    
        % \begin{figure}
        %     \CenterFloatBoxes
        %     \begin{floatrow}
        %     \ffigbox[\FBwidth]{
        %       \includegraphics[scale=0.30]{figures/runtimes/mini.pdf}
        %     }{
        %     \vspace{-1em}
        %       \caption{Convergence plots for our methods on \textit{mini}-ImageNet with a ResNet-18. Solid lines are averages, while shadows are 95\% confidence intervals. Time is in logarithmic scale.}
        %       \label{fig:convergence_methods}
        %     }
        %     \killfloatstyle
        %     \capbtabbox{
        %         \small
        %         \begin{tabular}{lcc}
        %             \multicolumn{3}{c}{\textbf{Runtimes}} \\
        %             \toprule
        %             Method & Param. & Infer./task (s) \\
        %             \toprule
        %             Simp.Shot \cite{simpleshot}& $\{\textbf{W}\}$ &  9.0 $e^{-3}$ \\
        %             % \midrule
        %             Lapl.Shot \cite{Laplacian}$^{\dagger}$ & $\{\textbf{W}\}$ & 1.2 $e^{-2}$ \\
        %             \rowcolor{Gray} TIM-ADM $^{\dagger}$ & $\{\textbf{W}\}$ & 1.2 $e^{-1}$\\
        %             \rowcolor{Gray} TIM-GD $^{\dagger}$ & $\{\textbf{W}\}$ & 2.2 $e^{+0}$\\
        %             Ent-min $^{\ddagger}$ \cite{dhillon2019baseline} & $\{\boldsymbol{\phi}, \textbf{W}\}$ & 2.1 $ e^{+1}$ \\
        %             \bottomrule
        %         \end{tabular}
        %     }{
        %       \caption{Inference runtime per task for a 5-shot 5-way task on mini-ImageNet with a WRN28-10 backbone. Methods marked with $^{\dagger}$ are transductive.}%
        %       \label{tab:runtimes}
        %     }
        %     \end{floatrow}
        % \end{figure}
        \begin{figure}[t]
            \centering
            \includegraphics[scale=0.4]{figures/runtimes/mini.pdf}
            \caption{Convergence plots for our methods on \textit{mini}-ImageNet with a ResNet-18. Solid lines are averages, while shadows are 95\% confidence intervals. Time is in logarithmic scale. \textbf{Left:} Evolution of the test accuracy during transductive inference. \textbf{Right:} Evolution of the mutual information between query features and predictions $\widehat{\mathcal{I}}(X_\mathcal{Q};Y_\mathcal{Q})$, computed as in Eq. (\ref{prior-aware-MI}), with $\alpha=1$.}
            \label{fig:convergence_methods}
        \end{figure}
        
        \begin{table}[t]
            \centering
                \begin{tabular}{lccc}
                    \multicolumn{4}{c}{\textbf{Run-times}} \\
                    \toprule
                    Method & Parameters & Transductive & Inference/task (s) \\
                    \toprule
                    SimpleShot \cite{simpleshot}& $\{\textbf{W}\}$ & \xmark & $9.0 \times 10^{-3}$ \\
                    \midrule
                    % LaplacianShot & $\{\textbf{W}\}$ & & $1.2 \times 10^{-2}$ \\
                    \rowcolor{Gray} TIM-ADM & $\{\textbf{W}\}$ & & $1.2 \times 10^{-1}$\\
                    \rowcolor{Gray} TIM-GD & $\{\textbf{W}\}$ & & $2.2 \times 10^{+0}$\\
                    Ent-min \cite{dhillon2019baseline} & $\{\boldsymbol{\phi}, \textbf{W}\}$ & \multirow{-4}{*}{\cmark} & $2.1 \times 10^{+1}$ \\
                    \bottomrule
                \end{tabular}
            \caption{Inference run-time per few-shot task for a 5-shot 5-way task on mini-ImageNet with a WRN28-10 backbone.}
            \label{tab:runtimes}
        \end{table}



==> Neurips 2021 (4)/legacy.tex <==
\subsection{Performance gain compare to baseline}
The gain in performance of classifier trained with negative random samples while varying number of shots and ways.

\subsection{Comparison to state-of-the-art}\label{sec:benchmark}
We report the performance of our network in comparison with state-of-the-art methods in both transductive and inductive settings.

\begin{table}
	\centering
	\caption{Comparison to the state-of-the-art methods on \textit{mini}-ImageNet, \textit{tiered}-Imagenet and CUB using \textbf{transductive} settings. Our results (yellow-shaded) are averaged over 10,000 episodes. "-" signifies the result is unavailable.}
	\begin{tabular}{lcccccccc}
		& &\multicolumn{2}{c}{\textbf{\textit{mini}-ImageNet}} & \multicolumn{2}{c}{\textbf{\textit{tiered}-ImageNet}} & \multicolumn{2}{c}{\textbf{CUB}} \\
		Method & Backbone & 1-shot & 5-shot & 1-shot & 5-shot & 1-shot & 5-shot\\
		\toprule
		RelatNet + T \cite{can} &  ResNet-12 & 52.4 & 65.4 & - & - & - & -\\
		ProtoNet + T \cite{can} & ResNet-12 & 55.2 & 71.1 & - & - & - & -\\
		MatchNet+T \cite{can} &  ResNet-12 & 56.3 & 69.8 & - & - & - & -\\
		TPN \cite{liu2018learning} & ResNet-12 & 59.5 & 75.7 & - & - & - & -\\
		TEAM \cite{team}&  ResNet-18 & 60.1 & 75.9 & - & - & - & -\\
		Ent-min \cite{dhillon2019baseline}& ResNet-12 & 62.4 & 74.5 & 68.4 & 83.4 & - & -\\
		CAN+T \cite{can}&  ResNet-12 & 67.2 & 80.6 & 73.2 & 84.9 & - & -\\
		LaplacianShot \cite{Laplacian} & ResNet-18 & 72.1 & 82.3 & 79.0 & 86.4 & 81.0 & 88.7 \\
		TIM-ADM & ResNet-18 & 73.6 & 85.0 & 80.0 & 88.5 & 81.9 & 90.7 \\
		TIM-GD & ResNet-18 & 73.9 & 85.0 & 79.9 & \textbf{88.5} & 82.2 & 90.8 \\
		\rowcolor{Yellow}  JSC  & ResNet-18 & 75.69 & 83.87 & 81.10 & 87.06 & - & - \\
		\rowcolor{Yellow} JSC  & ResNet-12 & 77.63 & 85.50 & 80.49 & 86.70 & - & - \\
		\toprule
		AWGIM \cite{guo2020attentive}&  WRN28-10 & 63.1 & 78.4 & 67.7 & 82.8 & - & -\\
		Ent-min \cite{dhillon2019baseline} & WRN28-10 & 65.7 & 78.4 & 73.3 & 85.5 & - & -\\
		SIB  \cite{hu2020empirical} & WRN28-10 & 70.0 & 79.2 & - & - & - & -\\
		BD-CSPN \cite{prototype}&  WRN28-10 & 70.3 & 81.9 & 78.7 & 86.92 & - & -\\
		LaplacianShot  \cite{Laplacian}  & WRN28-10 & 74.9 & 84.1 & 80.2 & 87.6 & - & -\\
		TIM-ADM & WRN28-10 & 77.5 & 87.2 & 82.0 & 89.7 & - & -\\
		TIM-GD & WRN28-10 & 77.8 & \textbf{87.4} & 82.1 & \textbf{89.8} & - & -\\
		\rowcolor{Yellow} JSC & WRN28-10 &  76.83 & 84.96 & 82.65 & 88.20 & - & -\\
		\rowcolor{Yellow} JSC (with Entropy) & WRN28-10 &  \textbf{78.00} & 86.20 & \textbf{83.66}  &  89.37& - & -\\
		\bottomrule
	\end{tabular}
	\label{tab:benchmark_results}
\end{table}

\begin{table}
	\newlength\wexp
	\settowidth{\wexp}{\textbf{\textit{mini}-ImageNet} $\rightarrow$ \textbf{CUB}}
	\centering
	\small
	\caption{The results for the domain-shift setting \textit{mini}-Imagenet $\rightarrow$ CUB. The results obtained by our models (gray-shaded) are averaged over 10,000 episodes.}
	\begin{tabular}{lcccc}
		% \begin{tabular}{lcccc*{2}{w{c}{\dimexpr.5\wexp-\tabcolsep}}}
		& & \multicolumn{1}{c}{\textbf{\textit{mini}-ImageNet} $\rightarrow$ \textbf{CUB}}\\
		Methods & Backbone & 5-shot\\
		\toprule
		MatchNet \cite{matching_net} & ResNet-18 & 53.1\\
		MAML \cite{maml} & ResNet-18 & 51.3 \\
		ProtoNet \cite{prototypical_nets} & ResNet-18 & 62.0 \\
		RelatNet \cite{relation_net} & ResNet-18 & 57.7 \\
		%  CL2N \cite{simpleshot} & ResNet-18 & 70.1 & 86.3 & 48.0 & 64.0 \\
		SimpleShot \cite{simpleshot} & ResNet-18 & 64.0 \\
		GNN \cite{tseng2020cross} & ResNet-10 & 66.9 \\
		Neg-Cosine \cite{liu2020negative} & ResNet-18 & 67.0 \\
		Baseline \cite{closer_look} & ResNet-18 & 65.6 \\
		LaplacianShot \cite{Laplacian} & ResNet-18 & 66.3 \\
		\rowcolor{Gray} TIM-ADM & ResNet-18 & 70.3 \\
		\rowcolor{Gray} TIM-GD & ResNet-18 & \textbf{71.0} \\
		\bottomrule
	\end{tabular}
	\label{tab:domin_shift_results}
\end{table}

\subsection{Imbalanced query set}

\subsection{Semi-supervised and transductive settings}

\subsection{Comparison with vanila k-means clustering} 

\subsection{Impact of domain-shift}   
Chen et al. \cite{closer_look} recently showed that the performance of most meta-learning methods may drop drastically when a domain-shift exists between the base training data and test data. Surprisingly, the simplest 
discriminative baseline exhibited the best performance in this case. Therefore, we evaluate our methods in this challenging scenario. To this end, we simulate a domain shift by training the feature encoder on \textit{mini}-Imagenet while evaluating the methods on \textit{CUB}, similarly to the setting introduced in \cite{closer_look}. TIM-GD and TIM-ADM beat previous methods by significant margins in the domain-shift scenario, consistently with our results in the standard few-shot benchmarks, thereby demonstrating an increased potential of applicability to real-world situations.

\subsection{Pushing the meta-testing stage}

Most few-shot papers only evaluate their method in the usual 5-way scenario. Nevertheless, \cite{closer_look} showed that meta-learning methods could be beaten by their discriminative baseline when more ways were introduced in each task. Therefore, we also provide results of our method in the more challenging 10-way and 20-way scenarios on \textit{mini}-ImageNet. These results, which are presented in \autoref{tab:more_ways}, show that TIM-GD outperforms other methods by significant margins, in both settings.
\begin{table}
	\centering
	\caption{Results for increasing the number of classes on \textit{mini}-ImageNet. The results obtained by our models (gray-shaded) are averaged over 10,000 episodes.}
	\small
	\begin{tabular}{lcccccccc}
		& & \multicolumn{2}{c}{10-way} & \multicolumn{2}{c}{20-way} \\
		Methods & Backbone & 1-shot & 5-shot & 1-shot & 5-shot\\
		\toprule
		MatchNet \cite{matching_net}& ResNet-18 & - & 52.3 & - & 36.8 \\
		ProtoNet \cite{prototypical_nets}& ResNet-18 & - & 59.2 & - & 45.0 \\
		RelatNet \cite{relation_net}& ResNet-18 & - & 53.9 & - & 39.2 \\
		SimpleShot \cite{simpleshot}& ResNet-18 & 45.1 & 68.1 & 32.4 & 55.4 \\
		Baseline \cite{closer_look}& ResNet-18 & - & 55.0 & - & 42.0 \\
		Baseline++ \cite{closer_look}& ResNet-18 & - & 63.4 & - & 50.9 \\
		\rowcolor{Gray} TIM-ADM & ResNet-18 & 56.0 & \textbf{72.9} & \textbf{39.5} & 58.8 \\
		\rowcolor{Gray} TIM-GD & ResNet-18 & \textbf{56.1} & 72.8 & 39.3 & \textbf{59.5} \\
		\bottomrule
	\end{tabular}
	\label{tab:more_ways}
\end{table}

\subsection{Ablation study}

\subsubsection{Influence of each term: }\label{sec:ablation_terms} 

\begin{table}[t]
	\small
	\centering
	\caption{Ablation study on the effect of each term in our loss in Eq. \eqref{eq:tim_objective}, when only the classifier weights are fine-tuned, i.e., updating only $\textbf{W}$, and when the whole network is fine-tuned, i.e., updating $\{\boldsymbol{\phi},\textbf{W}\}$. The results are reported for ResNet-18 as backbone. 
		The same term indexing as in Eq. \eqref{eq:tim_objective} is used here: $\widehat{\mathcal{H}}(Y_\mathcal{Q})$: Marginal entropy, $\widehat{\mathcal{H}}(Y_\mathcal{Q}|X_\mathcal{Q})$: Conditional entropy, $\mathrm{CE}$: Cross-entropy.}
	\resizebox{\textwidth}{!}{
		\begin{tabular}{ccccccccc}
			& & & \multicolumn{2}{c}{\textbf{\textit{mini}-ImageNet}} & \multicolumn{2}{c}{\textbf{\textit{tiered}-ImageNet}} & \multicolumn{2}{c}{\textbf{CUB}}\\
			Method & Param. & Loss & 1-shot & 5-shot & 1-shot & 5-shot & 1-shot & 5-shot \\
			\toprule
			\multirow{4}{*}{TIM-ADM} & \multirow{4}{*}{$\{\textbf{W}\}$} & $\mathrm{CE}$ & 60.0 & 79.6 & 68.0 & 84.6 & 68.6 & 86.4 \\
			& & $\mathrm{CE} + \widehat{\mathcal{H}}(Y_\mathcal{Q}|X_\mathcal{Q})$ & 36.0 & 77.0 & 48.1 & 82.5 & 48.5 & 86.5 \\
			& & $\mathrm{CE} - \widehat{\mathcal{H}}(Y_\mathcal{Q})$ & 66.7 & 82.0 & 74.0 & 86.5 & 74.2 & 88.3 \\
			& & $\mathrm{CE} - \widehat{\mathcal{H}}(Y_\mathcal{Q}) + \widehat{\mathcal{H}}(Y_\mathcal{Q}|X_\mathcal{Q})$ & \textbf{73.6} & \textbf{85.0} & \textbf{80.0} & \textbf{88.5} & \textbf{81.9} & \textbf{90.7} \\
			\bottomrule
	\end{tabular}}
	\label{tab:ablation_effect_terms}
\end{table}

\subsubsection{Different number of query images}

\subsubsection{Different number of finetuning steps}

\section{Conclusion and future work}


==> Neurips 2021 (4)/misc.tex <==
%% notations
\newcommand{\sect}[1]{Section~\ref{#1}}
\newcommand{\sects}[1]{Sections~\ref{#1}}
\newcommand{\eqn}[1]{Equation~\ref{#1}}
\newcommand{\eqns}[1]{Equations~\ref{#1}}
\newcommand{\fig}[1]{Figure~\ref{#1}}
\newcommand{\figs}[1]{Figures~\ref{#1}}
\newcommand{\tab}[1]{Table~\ref{#1}}
\newcommand{\tabs}[1]{Tables~\ref{#1}}

% personalized command
\newcommand{\best}[1]{\mathbf{\textcolor{blue}{{#1}}}}
\newcommand{\secondbest}[1]{\textcolor{blue}{{#1}}}
\newcommand{\algo}{\texttt{POODLE}\xspace}
\newcommand{\longalgo}{\textbf{P}enalizing \textbf{O}ut-\textbf{O}f-\textbf{D}istribution samp\textbf{LE}s}
\newcommand{\etal}[1]{{{#1}} \textit{et al.}}
\newcommand{\ie}{\emph{i.e.,}~}
\newcommand{\eg}{\emph{e.g.,}~}
\newcommand{\wrt}{\emph{w.r.t.}~}
\newcommand{\myparagraph}[1]{\vspace{-6pt}\paragraph{#1}}

%color
\usepackage[colorinlistoftodos, textwidth=30mm, shadow, textsize=small]{todonotes}
\definecolor{babyblue}{rgb}{0.54, 0.81, 0.94}
\definecolor{citrine}{rgb}{0.89, 0.82, 0.04}
\definecolor{misocolor}{rgb}{0.16,0.27,0.86}
\definecolor{jbcolor}{rgb}{0.9,0.4,0.2}
\definecolor{bernacolor}{rgb}{0.9608,0.4863,0.00}
\definecolor{carlcolor}{rgb}{0.0,0.9863,0.30}
\definecolor{grey}{rgb}{0.3, 0.3, 0.3}
\newcommand{\todom}[1]{\todo[color=misocolor!30]{#1}\xspace}
\newcommand{\todomi}[1]{\todo[inline,color=misocolor!30]{#1}}
\newcommand{\todoinline}[1]{\todo[inline,color=grey!30]{#1}}


\newcommand{\todoco}[1]{\todo[color=citrine!30]{#1}\xspace}
\newcommand{\todocoi}[1]{\todo[inline,color=citrine!30]{#1}\xspace}
\newcommand{\todojb}[1]{\todo[color=jbcolor!30]{#1}\xspace}
\newcommand{\todoberna}[1]{\todo[color=bernacolor!10]{#1}\xspace}
\newcommand{\todor}[1]{\todo[color=babyblue]{R\' emi: #1}\xspace}
\newcommand{\todori}[1]{\todo[inline,color=babyblue]{R\' emi: #1}\xspace}
\newcommand{\todofloriani}[1]{\todo[inline,color=grey!15]{Florian: #1}\xspace}
\newcommand{\carl}[1]{\todo[color=carlcolor!50]{#1}\xspace}


\definecolor{graphicbackground}{rgb}{0.96,0.96,0.8}
\definecolor{rouge1}{RGB}{226,0,38}  % red P
\definecolor{orange1}{RGB}{243,154,38}  % orange P
\definecolor{jaune}{RGB}{254,205,27}  % jaune P
\definecolor{blanc}{RGB}{255,255,255} % blanc P
\definecolor{rouge2}{RGB}{230,68,57}  % red S
\definecolor{orange2}{RGB}{236,117,40}  % orange S
\definecolor{taupe}{RGB}{134,113,127} % taupe S
\definecolor{gris}{RGB}{91,94,111} % gris S
\definecolor{bleu1}{RGB}{38,109,131} % bleu S
\definecolor{bleu2}{RGB}{28,50,114} % bleu S
\definecolor{vert1}{RGB}{133,146,66} % vert S
\definecolor{vert3}{RGB}{20,200,66} % vert S
\definecolor{vert2}{RGB}{157,193,7} % vert S
\definecolor{darkyellow}{RGB}{233,165,0}  % orange S
\definecolor{lightgray}{rgb}{0.9,0.9,0.9}
\definecolor{darkgray}{rgb}{0.6,0.6,0.6}
\definecolor{babyblue}{rgb}{0.54, 0.81, 0.94}
\definecolor{citrine}{rgb}{0.89, 0.82, 0.04}
\definecolor{misogreen}{rgb}{0.25,0.6,0.0}
\definecolor{PalePurp}{rgb}{0.66,0.57,0.66}
\definecolor{todocolor}{rgb}{0.66,0.99,0.99}
\definecolor{pearOne}{HTML}{2C3E50}
\definecolor{pearTwo}{HTML}{A9CF54}
\definecolor{pearTwoT}{HTML}{C2895B}
\definecolor{pearThree}{HTML}{E74C3C}
\colorlet{titleTh}{pearOne}
\colorlet{bull}{pearTwo}
\definecolor{pearcomp}{HTML}{B97E29}
\definecolor{pearFour}{HTML}{588F27}
\definecolor{pearFith}{HTML}{ECF0F1}
\definecolor{pearDark}{HTML}{2980B9}
\definecolor{pearDarker}{HTML}{1D2DEC}

% reference color
\hypersetup{
	colorlinks,
	citecolor=pearDark,
	linkcolor=pearThree,
	breaklinks=true,
	urlcolor=pearDarker}



==> Neurips 2021 (4)/shortcut.tex <==
% \newtheorem{defn}{Definition}
% \newtheorem{coro}{Corollary}
% \newtheorem{conjec}{Conjecture}
% \newtheorem{example}{Example}
% \newtheorem{Lem}{Lemma}
% \newtheorem{fact}{Fact}
% \newtheorem{prop}{{\bf Proposition}}

\renewcommand{\vec}[1]{\mathbf{#1}}

\newcommand{\base}{{\text{base}}}
\newcommand{\test}{{\text{test}}}

\newfloatcommand{capbtabbox}{table}[][\FBwidth]
% \newcommand{\ol}[1]{\overline{#1}}
% \newcommand{\mr}[1]{\mathrm{#1}}
% \newcommand{\tx}[1]{\textrm{#1}}
\newcommand{\tr}[1]{{#1}^\top}

% \newcommand{\Om}{\Omega}
% \newcommand{\UU}{\mathcal{U}}
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%
\newcommand{\CC}{\mathcal{C}}
\newcommand{\ceq}{\stackrel{\mathclap{\normalfont\mbox{c}}}{=}}
\newcommand{\defeq}{\vcentcolon=}
\newcommand{\x}{\bm{x}} % A vector-valued random variable.
\newcommand{\w}{\bm{w}} % A vector-valued random variable.
\newcommand{\p}{\bm{p}} % A vector-valued random variable.
\newcommand{\q}{\bm{q}} % A vector-valued random variable.
\newcommand{\cc}{\bm{c}} % A vector-valued random variable.
\newcommand{\y}{\bm{y}} % A vector-valued random variable.
\newcommand{\z}{\bm{z}} % A vector-valued random variable.
\newcommand{\Dcos}{D^{\text{cos}}}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
% \newcommand{\TT}{\mathcal{T}}
% \newcommand{\QQ}{\mathcal{Q}}
% \newcommand{\II}{\mathcal{I}}
% \newcommand{\FF}{\mathcal{F}}
\newcommand{\RR}{\mathbb{R}}
% \newcommand{\XX}{\mathcal{X}}
\newcommand{\HH}{\mathcal{H}}
% \newcommand{\DD}{\mathcal{D}}
% \newcommand{\BB}{\mathcal{B}}
% \newcommand{\SSS}{\mathcal{S}}
% \newcommand{\NN}{\mathcal{N}}
\newcommand{\LL}{\mathcal{L}}
% \newcommand{\PP}{\mathrm{Pr}}
% \newcommand{\ppi}{\vec \pi}
\newcommand{\pp}{\vec p}
% \newcommand{\qq}{\vec q}
% \newcommand{\dd}{\vec d}
% \newcommand{\cc}{\vec c}
% \newcommand{\CX}{\overline{X}}
% \newcommand{\ax}{\tilde x}
% \newcommand{\kk}{\vec k}
% \newcommand{\va}{\vec a}
% \newcommand{\hx}{\hat{\vec x}}
% \newcommand{\hy}{\widehat{\vec y}}
% \newcommand{\hu}{\widehat{\vec u}}
% \newcommand{\hW}{\widehat{W}}
% \newcommand{\hD}{\widehat{D}}
% \newcommand{\hL}{\widehat{L}}
% \newcommand{\hU}{\hat{U}}
% \newcommand{\hA}{\hat{A}}
% \newcommand{\hY}{\hat{Y}}
% \newcommand{\hV}{\hat{V}}
% \newcommand{\hS}{\hat{\Sigma}}
% \newcommand{\mx}{\overline{\vec x}}
% \newcommand{\hX}{\hat{X}}
% \newcommand{\yy}{\vec y}
\newcommand{\vo}{\vec 1}
% \newcommand{\vz}{\vec 0}
% \newcommand{\ww}{\vec w}
% \newcommand{\zz}{\vec z}
% \newcommand{\bb}{\beta}
% \newcommand{\s}{s}
% \newcommand{\ee}{\vec e}
\newcommand{\uu}{\vec u}
\newcommand{\xx}{\vec x}
\newcommand{\ff}{\vec f}
% \newcommand{\hh}{\vec h}
% \newcommand{\rr}{\vec r}
\newcommand{\aaa}{\boldsymbol{\alpha}}
% \newcommand{\bbb}{\boldsymbol{\beta}}
\newcommand{\ttt}{\boldsymbol{\theta}}
% \newcommand{\ssim}{\mathrm{sim}}
% \newcommand{\ssum}{\sum\limits}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
% \DeclareMathOperator*{\trace}{tr}
% \DeclareMathOperator*{\diag}{diag}
% \DeclareMathOperator*{\rank}{rank}

% %\def\Rt{\mathbb{R}^{2}}
% %\def\Rn{\mathbb{R}^{n}}
\def\real{{\mathbb R}}
% %\def\natural{{\mathbb N}}
% %\def\C{{\mathbf \chi}}
% %\newcommand{\vecprod}[2]{\left\langle#1,#2\right\rangle}

% \def\httilde{\mbox{\tt\raisebox{-.5ex}{\symbol{126}}}}

% \newcommand{\vnu}{\boldsymbol \nu}
% \newcommand{\lu}{\tr\uu L\uu}
% \newcommand{\lz}{\tr\zz L\zz}
% \newcommand{\vF}{\vec F}
% \newcommand{\vv}{\vec v}

==> legacy.tex <==
\subsection{Performance gain compare to baseline}
The gain in performance of classifier trained with negative random samples while varying number of shots and ways.

\subsection{Comparison to state-of-the-art}\label{sec:benchmark}
We report the performance of our network in comparison with state-of-the-art methods in both transductive and inductive settings.

\begin{table}
	\centering
	\caption{Comparison to the state-of-the-art methods on \textit{mini}-ImageNet, \textit{tiered}-Imagenet and CUB using \textbf{transductive} settings. Our results (yellow-shaded) are averaged over 10,000 episodes. "-" signifies the result is unavailable.}
	\begin{tabular}{lcccccccc}
		& &\multicolumn{2}{c}{\textbf{\textit{mini}-ImageNet}} & \multicolumn{2}{c}{\textbf{\textit{tiered}-ImageNet}} & \multicolumn{2}{c}{\textbf{CUB}} \\
		Method & Backbone & 1-shot & 5-shot & 1-shot & 5-shot & 1-shot & 5-shot\\
		\toprule
		RelatNet + T \cite{can} &  ResNet-12 & 52.4 & 65.4 & - & - & - & -\\
		ProtoNet + T \cite{can} & ResNet-12 & 55.2 & 71.1 & - & - & - & -\\
		MatchNet+T \cite{can} &  ResNet-12 & 56.3 & 69.8 & - & - & - & -\\
		TPN \cite{liu2018learning} & ResNet-12 & 59.5 & 75.7 & - & - & - & -\\
		TEAM \cite{team}&  ResNet-18 & 60.1 & 75.9 & - & - & - & -\\
		Ent-min \cite{dhillon2019baseline}& ResNet-12 & 62.4 & 74.5 & 68.4 & 83.4 & - & -\\
		CAN+T \cite{can}&  ResNet-12 & 67.2 & 80.6 & 73.2 & 84.9 & - & -\\
		LaplacianShot \cite{Laplacian} & ResNet-18 & 72.1 & 82.3 & 79.0 & 86.4 & 81.0 & 88.7 \\
		TIM-ADM & ResNet-18 & 73.6 & 85.0 & 80.0 & 88.5 & 81.9 & 90.7 \\
		TIM-GD & ResNet-18 & 73.9 & 85.0 & 79.9 & \textbf{88.5} & 82.2 & 90.8 \\
		\rowcolor{Yellow}  JSC  & ResNet-18 & 75.69 & 83.87 & 81.10 & 87.06 & - & - \\
		\rowcolor{Yellow} JSC  & ResNet-12 & 77.63 & 85.50 & 80.49 & 86.70 & - & - \\
		\toprule
		AWGIM \cite{guo2020attentive}&  WRN28-10 & 63.1 & 78.4 & 67.7 & 82.8 & - & -\\
		Ent-min \cite{dhillon2019baseline} & WRN28-10 & 65.7 & 78.4 & 73.3 & 85.5 & - & -\\
		SIB  \cite{hu2020empirical} & WRN28-10 & 70.0 & 79.2 & - & - & - & -\\
		BD-CSPN \cite{prototype}&  WRN28-10 & 70.3 & 81.9 & 78.7 & 86.92 & - & -\\
		LaplacianShot  \cite{Laplacian}  & WRN28-10 & 74.9 & 84.1 & 80.2 & 87.6 & - & -\\
		TIM-ADM & WRN28-10 & 77.5 & 87.2 & 82.0 & 89.7 & - & -\\
		TIM-GD & WRN28-10 & 77.8 & \textbf{87.4} & 82.1 & \textbf{89.8} & - & -\\
		\rowcolor{Yellow} JSC & WRN28-10 &  76.83 & 84.96 & 82.65 & 88.20 & - & -\\
		\rowcolor{Yellow} JSC (with Entropy) & WRN28-10 &  \textbf{78.00} & 86.20 & \textbf{83.66}  &  89.37& - & -\\
		\bottomrule
	\end{tabular}
	\label{tab:benchmark_results}
\end{table}

\begin{table}
	\newlength\wexp
	\settowidth{\wexp}{\textbf{\textit{mini}-ImageNet} $\rightarrow$ \textbf{CUB}}
	\centering
	\small
	\caption{The results for the domain-shift setting \textit{mini}-Imagenet $\rightarrow$ CUB. The results obtained by our models (gray-shaded) are averaged over 10,000 episodes.}
	\begin{tabular}{lcccc}
		% \begin{tabular}{lcccc*{2}{w{c}{\dimexpr.5\wexp-\tabcolsep}}}
		& & \multicolumn{1}{c}{\textbf{\textit{mini}-ImageNet} $\rightarrow$ \textbf{CUB}}\\
		Methods & Backbone & 5-shot\\
		\toprule
		MatchNet \cite{matching_net} & ResNet-18 & 53.1\\
		MAML \cite{maml} & ResNet-18 & 51.3 \\
		ProtoNet \cite{prototypical_nets} & ResNet-18 & 62.0 \\
		RelatNet \cite{relation_net} & ResNet-18 & 57.7 \\
		%  CL2N \cite{simpleshot} & ResNet-18 & 70.1 & 86.3 & 48.0 & 64.0 \\
		SimpleShot \cite{simpleshot} & ResNet-18 & 64.0 \\
		GNN \cite{tseng2020cross} & ResNet-10 & 66.9 \\
		Neg-Cosine \cite{liu2020negative} & ResNet-18 & 67.0 \\
		Baseline \cite{closer_look} & ResNet-18 & 65.6 \\
		LaplacianShot \cite{Laplacian} & ResNet-18 & 66.3 \\
		\rowcolor{Gray} TIM-ADM & ResNet-18 & 70.3 \\
		\rowcolor{Gray} TIM-GD & ResNet-18 & \textbf{71.0} \\
		\bottomrule
	\end{tabular}
	\label{tab:domin_shift_results}
\end{table}

\subsection{Imbalanced query set}

\subsection{Semi-supervised and transductive settings}

\subsection{Comparison with vanila k-means clustering} 

\subsection{Impact of domain-shift}   
Chen et al. \cite{closer_look} recently showed that the performance of most meta-learning methods may drop drastically when a domain-shift exists between the base training data and test data. Surprisingly, the simplest 
discriminative baseline exhibited the best performance in this case. Therefore, we evaluate our methods in this challenging scenario. To this end, we simulate a domain shift by training the feature encoder on \textit{mini}-Imagenet while evaluating the methods on \textit{CUB}, similarly to the setting introduced in \cite{closer_look}. TIM-GD and TIM-ADM beat previous methods by significant margins in the domain-shift scenario, consistently with our results in the standard few-shot benchmarks, thereby demonstrating an increased potential of applicability to real-world situations.

\subsection{Pushing the meta-testing stage}

Most few-shot papers only evaluate their method in the usual 5-way scenario. Nevertheless, \cite{closer_look} showed that meta-learning methods could be beaten by their discriminative baseline when more ways were introduced in each task. Therefore, we also provide results of our method in the more challenging 10-way and 20-way scenarios on \textit{mini}-ImageNet. These results, which are presented in \autoref{tab:more_ways}, show that TIM-GD outperforms other methods by significant margins, in both settings.
\begin{table}
	\centering
	\caption{Results for increasing the number of classes on \textit{mini}-ImageNet. The results obtained by our models (gray-shaded) are averaged over 10,000 episodes.}
	\small
	\begin{tabular}{lcccccccc}
		& & \multicolumn{2}{c}{10-way} & \multicolumn{2}{c}{20-way} \\
		Methods & Backbone & 1-shot & 5-shot & 1-shot & 5-shot\\
		\toprule
		MatchNet \cite{matching_net}& ResNet-18 & - & 52.3 & - & 36.8 \\
		ProtoNet \cite{prototypical_nets}& ResNet-18 & - & 59.2 & - & 45.0 \\
		RelatNet \cite{relation_net}& ResNet-18 & - & 53.9 & - & 39.2 \\
		SimpleShot \cite{simpleshot}& ResNet-18 & 45.1 & 68.1 & 32.4 & 55.4 \\
		Baseline \cite{closer_look}& ResNet-18 & - & 55.0 & - & 42.0 \\
		Baseline++ \cite{closer_look}& ResNet-18 & - & 63.4 & - & 50.9 \\
		\rowcolor{Gray} TIM-ADM & ResNet-18 & 56.0 & \textbf{72.9} & \textbf{39.5} & 58.8 \\
		\rowcolor{Gray} TIM-GD & ResNet-18 & \textbf{56.1} & 72.8 & 39.3 & \textbf{59.5} \\
		\bottomrule
	\end{tabular}
	\label{tab:more_ways}
\end{table}

\subsection{Ablation study}

\subsubsection{Influence of each term: }\label{sec:ablation_terms} 

\begin{table}[t]
	\small
	\centering
	\caption{Ablation study on the effect of each term in our loss in Eq. \eqref{eq:tim_objective}, when only the classifier weights are fine-tuned, i.e., updating only $\textbf{W}$, and when the whole network is fine-tuned, i.e., updating $\{\boldsymbol{\phi},\textbf{W}\}$. The results are reported for ResNet-18 as backbone. 
		The same term indexing as in Eq. \eqref{eq:tim_objective} is used here: $\widehat{\mathcal{H}}(Y_\mathcal{Q})$: Marginal entropy, $\widehat{\mathcal{H}}(Y_\mathcal{Q}|X_\mathcal{Q})$: Conditional entropy, $\mathrm{CE}$: Cross-entropy.}
	\resizebox{\textwidth}{!}{
		\begin{tabular}{ccccccccc}
			& & & \multicolumn{2}{c}{\textbf{\textit{mini}-ImageNet}} & \multicolumn{2}{c}{\textbf{\textit{tiered}-ImageNet}} & \multicolumn{2}{c}{\textbf{CUB}}\\
			Method & Param. & Loss & 1-shot & 5-shot & 1-shot & 5-shot & 1-shot & 5-shot \\
			\toprule
			\multirow{4}{*}{TIM-ADM} & \multirow{4}{*}{$\{\textbf{W}\}$} & $\mathrm{CE}$ & 60.0 & 79.6 & 68.0 & 84.6 & 68.6 & 86.4 \\
			& & $\mathrm{CE} + \widehat{\mathcal{H}}(Y_\mathcal{Q}|X_\mathcal{Q})$ & 36.0 & 77.0 & 48.1 & 82.5 & 48.5 & 86.5 \\
			& & $\mathrm{CE} - \widehat{\mathcal{H}}(Y_\mathcal{Q})$ & 66.7 & 82.0 & 74.0 & 86.5 & 74.2 & 88.3 \\
			& & $\mathrm{CE} - \widehat{\mathcal{H}}(Y_\mathcal{Q}) + \widehat{\mathcal{H}}(Y_\mathcal{Q}|X_\mathcal{Q})$ & \textbf{73.6} & \textbf{85.0} & \textbf{80.0} & \textbf{88.5} & \textbf{81.9} & \textbf{90.7} \\
			\bottomrule
	\end{tabular}}
	\label{tab:ablation_effect_terms}
\end{table}

\subsubsection{Different number of query images}

\subsubsection{Different number of finetuning steps}

\section{Conclusion and future work}

